Towards Sparsification of Graph Neural Networks

As real-world graphs expand in size, larger GNN models with billions of parameters are deployed. High parameter count in such models makes training and inference on graphs expensive and challenging. To reduce the computational and memory costs of GNNs, optimization methods such as pruning the redundant nodes and edges in input graphs have been commonly adopted. However, model compression, which directly targets the sparsification of model layers, has been mostly limited to traditional Deep Neural Networks (DNNs) used for tasks such as image classification and object detection. In this paper, we utilize two state-of-the-art model compression methods (1) train and prune and (2) sparse training for the sparsification of weight layers in GNNs. We evaluate and compare the efficiency of both methods in terms of accuracy, training sparsity, and training FLOPs on real-world graphs. Our experimental results show that on the ia-email, wiki-talk, and stackoverflow datasets for link prediction, sparse training with much lower training FLOPs achieves a comparable accuracy with the train and prune method. On the brain dataset for node classification, sparse training uses a lower number FLOPs (less than 1/7 FLOPs of train and prune method) and preserves a much better accuracy performance under extreme model sparsity.

==> Sections/long_admm_copy.tex <==
\subsection{Weight Pruning Using ADMM and SLR}

\textcolor{red}{copied, re-write@deniz. } Consider a FNN with $N$ layers, where the weights at layer $n$ are denoted by ${{\bf W}}_{n}$ for $n \in \{1,2,...,N\}$. In the ADMM and SLR training, the loss function can be defined as  $ f \big( {\bf{W}}_{n}\big) +
     \sum_{n=1}^{N} g_{n}({\bf{W}}_{n})$,
for each layer $n$, where the first term represents the nonlinear smooth loss function and the second term represents the non-differentiable "cardinality" penalty term~\cite{zhang2018systematic} that is defined as:

\begin{eqnarray*}g_{n}({\bf{W}}_{n})=
\begin{cases}
 0 & \text {if } \mathrm{card}({\bf{W}}_{n})\le l_{n}, \; n = 1, \ldots, N, \\
 +\infty & \text {otherwise. } 
\end{cases}
\end{eqnarray*}

The indicator function $g_{n}(\cdot)$ ensures that the number of nonzero weights are less than or equal to the predefined number $l_n$ within each layer $n$. The objective of ADMM and SLR training is to minimize the loss function. However, because the loss function is subject to constraints on the cardinality of weights, it cannot be solved in its entirety. ADMM and SLR techniques decompose the loss problem into 2 smaller subproblems by introducing duplicate variables  ${\bf{W}}_{n}={\bf{Z}}_{n}$ and rewriting the problem as $\underset{ {\bf{W}}_{n}}{\text{min}}
 f \big( {\bf{W}}_{n} \big)+\sum_{n=1}^{N} g_{n}({\bf{Z}}_{n}) \label{losscardinality}$. The \textit{Augmented} Lagrangian function ~\cite{Boyd2011DistributedOA,zhang2018systematic} of this problem can be written as:
\begin{equation}
\begin{aligned}
 L_{\rho} &   \big( {\bf{W}}_{n}, {\bf{Z}}_{n} , {\bf{\Lambda}}_{n}  \big) = 
   f \big( {\bf{W}}_{n} \big) \label{relaxedproblem}
 + \sum_{n=1}^{N} g_{n}({\bf{Z}}_{n})
\\  & +\sum_{n=1}^{N} \mathrm{tr} [{\bf{\Lambda}}_{n}^T({\bf{W}}_{n}-{\bf{Z}}_{n}) ]
 + \sum_{n=1}^{N} \frac{\rho}{2} \| {\bf{W}}_{n}-{\bf{Z}}_{n} \|_{F}^{2},
\end{aligned}
\end{equation}
where ${\bf{\Lambda}}_{n}$ are dual variables corresponding to constraints ${\bf{W}}_{n}={\bf{Z}}_{n}$. The positive scalar $\rho$ is the penalty coefficient, $\mathrm{tr}(\cdot)$ denotes the trace, and $ \| \cdot \|_{F}^{2}$ denotes the Frobenius norm. 

After the decomposition of the problem, the subproblems are solved iteratively in 2 steps: 
\begin{enumerate}
    \item Solve ``Loss Function" subproblem for ${\bf{W}}_{n}$ by using stochastic gradient descent.
    \item Solve "Cardinality" subproblem for ${\bf{Z}}_{n}$ through pruning by using projections onto discrete subspace.
\end{enumerate}

\textbf{Alternating Direction Method of Multipliers.}
ADMM-based weight pruning defines  ${\bf U}_{n} = (1/\rho) {\bf{\Lambda}}_{n}$. Then, the first subproblem at iteration $k$ can be equivalently written as
\begin{equation}\label{eq:admm_loss}
\begin{aligned}
\underset{ {\bf{W}}_{n}}{\text{min}} \
 f \big( {\bf{W}}_{n} \big)+\sum_{n=1}^{N} \frac{\rho}{2} \| {\bf{W}}_{n}-{\bf{Z}}_{n}^{k} + {\bf{U}}_{n}^{k} \|_{F}^{2},
 \end{aligned}
\end{equation}

\noindent where the first term is the differentiable loss function of the DNN, while the other quadratic terms are differentiable and
convex. Therefore, the first subproblem (Eq. \ref{eq:admm_loss})
can be solved by using stochastic gradient descent (SGD)\cite{bottou2010large}. The second subproblem is
\begin{equation}\label{eq:admm_card}
\begin{aligned}
\underset{ {\bf{Z}}_{n}}{\text{min}} \
  g_{n}({\bf{Z}}_{n}) +\sum_{n=1}^{N} \frac{\rho}{2} \| {\bf{W}}_{n}^{k+1}-{\bf{Z}}_{n} + {\bf{U}}_{n}^{k} \|_{F}^{2},
 \end{aligned}
\end{equation}

The globally optimal solution
of this can be derived using the Euclidean projection of ${\bf{W}}_{n}^{k+1}$ and ${\bf{U}}_{n}^{k}$ onto the set ${\bf{S}}_{n}= \{{\bf{W}}_{n}\mid \mathrm{card}({\bf{W}}_{n})\le l_{n}  \}, n=1,\dots,N$. After both subproblems (Eq. \ref{eq:admm_loss} and \ref{eq:admm_card}) are solved, the dual variables are updated as ${\bf{U}}_{n}^{k+1} = {\bf{U}}_{n}^{k} + {\bf{W}}_{n}^{k+1} - {\bf{Z}}_{n}^{k+1}$ 
and this completes one iteration in ADMM regularization. 

\textbf{Surrogate Lagrangian Relaxation.}
At iteration $k$, for given values of multipliers ${\bf{\Lambda}}_{n}^k$, the first subproblem tries to minimize the Lagrangian function, while keeping ${\bf{Z}}_{n}$ at previously obtained values ${\bf{Z}}_{n}^{k-1}$ as

\begin{equation}
\begin{aligned}
 \min_{ {\bf{W}}_{n}} L_{\rho} &   \big( {\bf{W}}_{n}, {\bf{Z}}_{n}^{k-1} , {\bf{\Lambda}}_{n} \big). \label{slr_loss}
\end{aligned}
\end{equation}

Similar to ADMM, this subproblem can be solved using SGD. However, differently from ADMM, an additional "surrogate" optimality condition\cite{Bragin2015SLR} for updating the multipliers is used to ensure that multipliers' updating directions are "proper" as follows 
  \begin{equation}
% \begin{align}
\label{SOC1}
L_{\rho} \big({\bf{W}}_{n}^{k}, {\bf{Z}}_{n}^{k-1}, {\bf{\Lambda}}_{n}^{k} \big) < 
L_{\rho} \big({\bf{W}}_{n}^{k-1}, {\bf{Z}}_{n}^{k-1}, {\bf{\Lambda}}_{n}^{k} \big)
% \nonumber
% \end{align}
\end{equation}

If this condition is satisfied, multipliers are updated as ${\bf{\Lambda}'}_{n}^{k+1}: = {\bf{\Lambda}}_{n}^{k}+ s'^k({\bf{W}}_{n}^{k}-{\bf{Z}}_{n}^{k-1})$, where the stepsizes are calculated as follows



\begin{equation*}
\begin{aligned}
s'^{k} =& \alpha^{k} \frac{s^{k-1}||{\bf{W}}^{k-1}-{\bf{Z}}^{k-1}||}{||{\bf{W}}^{k}-{\bf{Z}}^{k-1}||}. \label{step1a}
\end{aligned}
\end{equation*}

The stepsize parameter can be defined as $\alpha^{k} = 1 - (1 / (M \times k^{(1-\frac{1}{k^r})}))$ for
 $M > 1$, $0 < r < 1$.



The second subproblem for cardinality is solved with respect to ${\bf{Z}}_{n}$ while fixing other variables at values ${\bf{W}}_{n}^k$ as  
\begin{equation}
\begin{aligned}
 \min_{ {\bf{Z}}_{n}} L_{\rho} &   \big( {\bf{W}}_{n}^k, {\bf{Z}}_{n}, {\bf{\Lambda}'}_{n}^{k+1} \big). \label{cardinalitysubproblem}
\end{aligned}
\end{equation}

The globally optimal solution to this problem is the same as ADMM where it is achieved through pruning using the Euclidean projection of ${\bf{W}}_{n}^{k}$ and ${\bf{\Lambda}'}_{n}^{k+1}$ onto discrete subspace. Again, in order to ensure that the multipliers' updating directions are proper, another "surrogate" optimality condition needs to be satisfied:
  \begin{equation}
% \begin{align}
\label{SOC}
 L_{\rho} \big({\bf{W}}_{n}^{k} , {\bf{Z}}_{n}^{k}, {\bf{\Lambda}'}_{n}^{k+1}  \big) < 
 L_{\rho} \big({\bf{W}}_{n}^{k} , {\bf{Z}}_{n}^{k-1} , {\bf{\Lambda}'}_{n}^{k+1} \big)
%  \nonumber
% \end{align}
\end{equation}

If this condition is not satisfied, then both subproblems are solved again by using the latest available values for  ${\bf{W}}_{n} $ and  ${\bf{Z}}_{n}$. However, if the condition is satisfied, multipliers are updated as ${\bf{\Lambda}}_{n}^{k+1}: = {\bf{\Lambda}'}_{n}^{k+1}+ s^k({\bf{W}}_{n}^{k}-{\bf{Z}}_{n}^{k})$ where the stepsizes are calculated as follows 

\begin{equation*}
\begin{aligned}
s^{k} =& \alpha^{k} \frac{s'^{k}||{\bf{W}}^{k-1}-{\bf{Z}}^{k-1}||}{||{\bf{W}}^{k}-{\bf{Z}}^{k}||}, \label{step1b}
\end{aligned}
\end{equation*}


Overall, SLR follows a similar approach to ADMM but additionally, it allows efficient subproblem solution coordination using (1) stepsizes approaching zero and (2) the satisfaction of surrogate optimality conditions ensuring updates to multipliers are assigned along correct directions. Since it supports independent and systematic adjustment of the penalty coefficient and stepsizes, model parameters obtained by SLR are much closer to their optimal values compared to ADMM, which does not support the adjustment of stepsizes without leading to slower convergence. The SLR weight pruning method has been shown to have faster convergence compared to ADMM and therefore, reduce the overall training time \cite{Gurevin2021EnablingRD}. 

\begin{figure*}[htpb!]
    %  \vspace{-.1in}
 \includegraphics[width = 0.94\linewidth]{Figs/training_process.pdf}
     \caption{Sparse training process for pattern pruning.}
    %  \vspace{-3mm}
     \label{fig:sparetraining}
\end{figure*}

